Dissecting Pruned Neural Networks

Pruning is a standard technique for removing unnecessary structure from a neural network to reduce its storage footprint, computational demands, or energy consumption. Pruning can reduce the parameter-counts of many state-of-the-art neural networks by an order of magnitude without compromising accuracy, meaning these networks contain a vast amount of unnecessary structure. In this paper, we study the relationship between pruning and interpretability. Namely, we consider the effect of removing unnecessary structure on the number of hidden units that learn disentangled representations of human-recognizable concepts as identified by network dissection. We aim to evaluate how the interpretability of pruned neural networks changes as they are compressed. We find that pruning has no detrimental effect on this measure of interpretability until so few parameters remain that accuracy beings to drop. Resnet-50 models trained on ImageNet maintain the same number of interpretable concepts and units until more than 90% of parameters have been pruned.

==> methodology.tex <==
\section{Methodology}

\textbf{Network.}
We study a ResNet-20~\citep{he_resnet_2015} trained on CIFAR-10~\citep{krizhevsky_cifar_2009}.
We use a standard implementation provided with TensorFlow, available online~\footnote{\url{https://github.com/tensorflow/models/tree/v1.13.0/official/resnet}}.
This implementation trains for $182$ epochs, using an initial learning rate of $0.1$, decaying by a factor of $10$ at epochs $91$ and $136$.
The network trains to \NA{XX.X\%} accuracy on CIFAR10.

\textbf{Fine-tuning experiments.}
There several hyperparameters that must be chosen when pruning with fine-tuning, namely the number of epochs $x$ for which fine-tuning will occur and the learning rate schedule during that phase.
In our experiments, we explore many values of $x$, which controls the cost of obtaining the final, pruned network (Criterion 1).
We follow the standard practice from \NA{CITE MANY PAPERS} to fine-tune using the final learning rate from the original training phase.

\textbf{Rewinding/replaying experiments.}
Rewinding includes only one hyperparameter: the number of epochs $x$ that the network should be rewound.
For example, consider a network that is normally trained for $T$ epochs.
We would train the network for the original $T$ epochs, prune, rewind the weights to their values at epoch $T - x$, and replay the remaining $x$ epochs of training on the pruned network.
When rewinding, the learning rate schedule is accordingly rewound to the same epoch.

We also consider rewinding with \emph{abbreviated replaying} in which we reduce the number of training epochs that occur during the replaying phase.
\citet{frankle_lottery_2019} observe that the subnetworks found using Algorithm \ref{alg:rewind} require fewer training steps than the original network to reach accuracy milestones.
We hypothesize that we can exploit this effect by replaying for fewer iterations than the original network was trained, potentially reducing the overall cost of finding a pruned network.
